Analyzing Coherency in Facet-based Clarification Prompt Generation for Search

Clarifying user's information needs is an essential component of modern search systems. While most of the approaches for constructing clarifying prompts rely on query facets, the impact of the quality of the facets is relatively unexplored. In this work, we concentrate on facet quality through the notion of facet coherency and assess its importance for overall usefulness for clarification in search. We find that existing evaluation procedures do not account for facet coherency, as evident by the poor correlation of coherency with automated metrics. Moreover, we propose a coherency classifier and assess the prevalence of incoherent facets in a well-established dataset on clarification. Our findings can serve as motivation for future work on the topic.

==> definitions.tex <==
\newcommand{\todop}[1]{\textcolor{blue}{[Silvia]: #1}}
\newcommand{\todoi}[1]{\textcolor{orange}{[Ivan]: #1}}
\newcommand{\tocheck}[1]{\textcolor{teal}{[To check]: #1}}
\newcommand{\maybe}[1]{\textcolor{gray}{#1}}
\newcommand{\todo}[1]{\textcolor{red}{#1}}

\acrodef{CIS}{conversational information seeking}
\acrodef{IR}{information retrieval}
\acrodef{NLP}{natural language processing}

\acrodef{LLM}{large language model}
\acrodefplural{LLM}{large language models}

\newcommand{\ourMethod}[0]{\textit{OurMethod}\xspace}

